Merlin:Empowering Multimodal LLMs with Foresight Minds

Humans possess the remarkable ability to foresee the future to a certain extent based on present observations, a skill we term as foresight minds. However, this capability remains largely under explored within existing Multimodal Large Language Models (MLLMs), hindering their capacity to learn the fundamental principles of how things operate and the intentions behind the observed subjects. To address this issue, we introduce the integration of future modeling into the existing learning frameworks of MLLMs. By utilizing the subject trajectory, a highly structured representation of a consecutive frame sequence, as a learning objective, we aim to bridge the gap between the past and the future. We propose two innovative methods to empower MLLMs with foresight minds, Foresight Pre-Training (FPT) and Foresight Instruction-Tuning (FIT), which are inspired by the modern learning paradigm of LLMs. Specifically, FPT jointly training various tasks centered on trajectories, enabling MLLMs to learn how to attend and predict entire trajectories from a given initial observation. Then, FIT requires MLLMs to first predict trajectories of related objects and then reason about potential future events based on them. Aided by FPT and FIT, we build a novel and unified MLLM named Merlin that supports multi-images input and analysis about potential actions of multiple objects for the future reasoning. Experimental results show Merlin powerful foresight minds with impressive performance on both future reasoning and visual comprehension tasks.

==> Tabs/ablation_future.tex <==
\begin{table}[h]
  \centering
  \small
  \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{@{}p{.8em}@{}ccccccc@{}}
  % \setlength{\tabcolsep}{3.5pt}
  % \begin{tabular}{ccccccc}
    \toprule
    Methods & MiniGPT-4-13B & mPLUG-Owl & Shikra & Kosmos-2 & Otter-I & Merlin \\
    \midrule
    Acc. & 21.4 & 28.6 & 42.9 & 52.4 & 54.8 & \textcolor{red}{XXX} \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Comparisons with future prediction.}}
\label{tab:future_prediction}
\end{table} 

==> Tabs/ablation_merlin.tex <==
\begin{table*}[t]
  \centering
\small
  \caption{\textbf{Ablation study of the proposed strategies in Merlin.} The resulting Merlin that combines PNF and T-CoT is highlighted in \colorbox{aliceblue!60}{violet} (PNF: Predicting Next Frame, T-CoT: Trajectory Chain-of-Thought). We mainly report the AO score of GOT10k and the metric of identity reasoning (Identity Rea), future prediction (Future Pre) and overall score in MMBench.}
  \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{@{}p{.8em}@{}lc cccccc| cc c cccc@{}}
    \toprule
     &&& \multicolumn{2}{c}{Foresight Pre-Training} && \multicolumn{2}{c}{Foresignt Instruction-Tuning} &&   \multicolumn{1}{c}{GOT10K} && \multicolumn{2}{c}{Future Reasoning} \\
    \cmidrule{3-5}
    \cmidrule{7-8}
    \cmidrule{10-10}
    \cmidrule{12-13}
	  & Method && Image-Text Pair & FPT-Data && LLaVA-665K~\cite{llava1.5} & FIT-Data && \textbf{AO} && \textbf{Average$_{dev}$} & \textbf{Average$_{test}$} \\
    \midrule
	  % \rownumber{1}&	  Base && \xmark & \xmark && \Checkmark & \xmark && - &&  & \\
	  \rownumber{1}&Base	   && \Checkmark & \xmark && \Checkmark & \xmark && - && 59.5 &  \\
	  \rownumber{2}&	   && \Checkmark & \xmark && \Checkmark & \Checkmark && - && 60.7 &  \\
        \rownumber{3}&	   && \xmark & \Checkmark && \Checkmark & \Checkmark && 15.5 && 52.8 &  \\
        \rownumber{4}&	   && \Checkmark & \Checkmark && \Checkmark & \xmark && 51.4 && 61.2 &  \\
	  \rowcolor{aliceblue!60} \rownumber{5}&	   Merlin && \Checkmark & \Checkmark && \Checkmark & \Checkmark && 51.4 && 64.4 &  \\
    \bottomrule
  \end{tabular}
  % \vspace{-1mm}
\label{tab:strategies}
\end{table*} 

==> Tabs/ablation_proj.tex <==
\begin{table}[t]
  \centering
  \scalebox{1.0}{
\small
%   \setlength{\tabcolsep}{3pt}
  \begin{tabular}{@{}ccc |cc@{}}
    \toprule
      Projector& Token Num && MMBench & MMVet \\
    \midrule
      Linear        & 1024 && \bf 21.9 & \bf 16.7\\
      Cross-attention            & 256 && 16.9 & 14.8 \\
      Convolution            & 256 && 16.9 & 14.8 \\
    \bottomrule
  \end{tabular}}
  \caption{\textbf{Experimental results of using different projectors.}}
  \label{tab:proj}
\end{table}





==> Tabs/vltask.tex <==
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison with SOTA methods on main MLLM benchmarks.} Res, PT, IT indicate input image resolution, the number of samples in pretraining and instruction tuning stage, respectively. For VQA tasks, we mainly choose VQA-v2~\cite{goyal2017vqav2}; GQA~\cite{hudson2019gqa}; VisWiz~\cite{gurari2018vizwiz}; VQA$^\text{T}$: TextVQA~\cite{singh2019textvqa} to evaluate the model; For the hallucination (Hall.) evaluation, we choose POPE~\cite{li2023pope} benchmark; For general evaluation, we mainly choose MMB: MMBench~\cite{liu2023mmbench}; MMB$^\text{CN}$: MMBench-Chinese~\cite{liu2023mmbench}; MM-Vet~\cite{yu2023mmvet}. We further select future prediction metric of MMBench to reflect the feature reasoning ability of the model. $^*$The training images of the datasets are observed during training. $^\dagger$Includes in-house data that is not publicly accessible.}
\scalebox{0.745}{
\begin{tabular}{l l p{5mm}p{7mm}p{7mm} c  p{8mm}p{8mm}p{8mm}p{8mm} c  p{8mm} c p{8mm} p{9mm} p{9mm} l l p{9mm}}
\toprule[.9pt]
&&&&&& \multicolumn{4}{c}{\textbf{VQA Task}} && \multicolumn{1}{c}{\textbf{Hall.}} && \multicolumn{4}{c}{\textbf{Generalist}} && \multicolumn{1}{c}{\textbf{Future}} \\
    \cmidrule{7-10}
    \cmidrule{12-12}
    \cmidrule{14-17}
    \cmidrule{19-19}
\textbf{Method} & LLM & Res. & PT & IT && VQA$^\text{v2}$ & GQA & VisWiz & VQA$^\text{T}$ && POPE && MMB & MMB$^\text{CN}$ & LLaVA$^\text{W}$ & MM-Vet && F Pre. \\
\midrule
BLIP-2 & Vicuna-13B & 224 & 129M & - && 41.0 & 41 & 19.6 & 42.5 && \underline{85.3} && -- & -- & 38.1 & 22.4 && --\\
InstructBLIP & Vicuna-7B & 224 & 129M & 1.2M && -- & 49.2 & 34.5 & 50.1 && -- && 36 & 23.7 & 60.9 & 26.2 && --\\
InstructBLIP & Vicuna-13B & 224 & 129M & 1.2M && -- & 49.5 & 33.4 & 50.7 && 78.9 && 44.0 & -- & 58.2 & 25.6 && 19.0\\
Shikra & Vicuna-13B & 224 & 600K & 5.5M && 77.4$^*$ & -- & -- & -- && -- && 58.8 & -- & -- & -- && 42.9\\
IDEFICS-9B & LLaMA-7B & 224 & 353M & 1M && 50.9 & 38.4 & 35.5 & 25.9 && -- && 48.2 & 25.2 & -- & -- && --\\
IDEFICS-80B & LLaMA-65B & 224 & 353M & 1M && 60.0 & 45.2 & 36.0 & 30.9 && -- && 54.5 & 38.1 & -- & -- && --\\
Qwen-VL & Qwen-7B & 448 & 1.4B$^\dagger$ & 50M$^\dagger$ && \underline{78.8}$^*$ & 59.3$^*$ & 35.2 & \textbf{63.8} && -- && 38.2 & 7.4  & -- & -- && --\\
Qwen-VL-Chat & Qwen-7B & 448 & 1.4B$^\dagger$ & 50M$^\dagger$ && 78.2$^*$ & 57.5$^*$ & 38.9 & \underline{61.5} && -- && 60.6 & 56.7 & -- & -- && --\\
LLaVA-1.5 & Vicuna-7B & 336 & 558K & 665K && \underline{78.5}$^*$ & \underline{62.0}$^*$ & \underline{50.0} & 58.2 && \textbf{85.9} && \underline{64.3} & \underline{58.3} & \underline{63.4} & \underline{30.5} && --\\
\midrule
\rowcolor{aliceblue!60}
\textbf{Merlin} & Vicuna-7B & 448 & \textbf{30M} & \textbf{665K} && \underline{80.5}$^*$ & \underline{60.4}$^*$ & \textbf{50.4} & 54.8 && \textbf{91.9} && \underline{69.2} & \underline{60.3} & \underline{66.4} & \underline{40.5} && -\\
\bottomrule[.9pt]
\end{tabular}
}
% \vspace{-1mm}
% \vspace{-6mm}
\label{tab:vltask}
\end{table*}
